Transient Structure in the Non-linear Superradiance Regime of Widely Doppler Broadened Media

We investigate transient radiation processes in the non-linear superradiance (SR) regime of the Doppler broadened Maxwell-Bloch equations when the velocity distribution is of total bandwidth greatly exceeding that of the transient process itself. We demonstrate the formation of global polarisation phase correlation and the quenching of temporal structure if a smooth distribution is inverted above the critical threshold required to enter the non-linear SR regime. We propose candidate stochastic velocity distributions capable of sustaining finite temporal structure in the non-linear emission process. We develop a novel algorithm for simulating the Doppler broadened Maxwell-Bloch equations which is $O(n)$ complex in the number of velocity channels $n$ whenever the emerging polarisation correlation is of moderate bandwidth, and we apply it to a stochastic velocity distribution in order to demonstrate sustained delay and duration of peak intensity in the widely Doppler broadened limit. We discuss the transverse inversion process and recognise an autoregulation mechanism on the number of molecules cooperatively participating in SR emission. This mechanism has the effect of limiting the temporal duration of the intensity pulse to a lower bound proportional to the length of the sample, which we confirm through simulation.

==> sections/999_archive.tex <==
% \documentclass[../main-wdb-sr.tex]{subfiles}
% \graphicspath{{\subfix{../figs/}}}
% \begin{document}

\subsubsection{Velocity distribution edge effects and periodic coupling in the supplementary fields algorithm}\label{subsubsec:theory-sfalg-pdc}

The simulations of Section \ref{subsec:swept-comb} will form the foundation of our understanding of a continuum distribution's ability to sustain (or not sustain) SR transient structure, but remain extremely narrow in velocity extent. In Section \ref{sec:cont} we will model WDB distributions and the potential development of SR processes deeply interior to a realistic continuum distribution; however, even these distributions will remain orders of magnitude smaller in velocity extent than any realistic gas. In order to ensure that our simulations realistically model the far interior of an actual velocity distribution, then, we should ensure that artifacts of our necessary truncation to a manageable total velocity extent will not corrupt our results.

Artificial behaviour in a finite velocity distribution occurs near the velocity boundaries, where velocity channels are coupled on only one ``side''; i.e., the leading edge of the velocity distribution at $\omega_\textrm{max}$ sees no adjacent channels for $\omega > \omega_\textrm{max}$ and the trailing edge at $\omega_\textrm{min}$ sees no adjacent channels for $\omega < \omega_\textrm{min}.$ A natural intuitive resolution to this nonphysical edge configuration is to introduce periodic boundary conditions to the velocity distribution; i.e., to couple the leading edge of the distribution to the trailing edge. We herein refer to such a configuration as periodic distribution coupling (PDC).

Implementing PDC on the velocity distribution is not a trivial mathematical task in either the CTD algorithm nor in the IF algorithm. The SF algorithm, however, provides a natural framework for coupling the leading edge of the distribution to the trailing edge. When propagating electric field modes near $\bar{\mathcal{E}}_{\omega_\textrm{min}}$ in $z$ via equation \eqref{eq:MB_TD-3_kernel} we make the replacement $\left[ F \bar{\mathcal{P}}\right] \left(\omega = \omega_\textrm{min} - \eta\right) \rightarrow \left[ F \bar{\mathcal{P}}\right] \left(\omega = \omega_\textrm{max} - \eta\right)$ for any $\eta$ establishing an integrand below $\omega_\textrm{min}$; similarly, for propagating modes near $\bar{\mathcal{E}}_{\omega_\textrm{max}}$ we make the replacement $\left[ F \bar{\mathcal{P}}\right] \left(\omega_\textrm{max} + \eta\right) \rightarrow \left[ F \bar{\mathcal{P}}\right] \left(\omega_\textrm{min} + \eta\right)$. This simplicity of PDC implementation is an additional advantage of the SF algorithm. Of course, it is only reasonable to implement PDC when the kernel width $\delta$ is much less than the total width of the distribution. The PDC configuration is depicted schematically in Figure \ref{fig:periodic_coupling}.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{pdc_visualisation.eps}
    \caption{Schematic of the PDC implementation. The ``chain links'' depict some particular $\textrm{LMI}^\textrm{SF}$ approximation interaction extent $\pm \delta/2$, which should always be much less than the total distribution width.}
    \label{fig:periodic_coupling}
\end{figure}

\subsubsection{First experiment: well below the critical threshold}\label{subsubsec:weaksrcomb}

Our first experiment begins with 11 samples each possessing an initial population inversion of $3.0\times {10}^{-6} \textrm{ m}^{-3}$ and separated by $\Delta v_\textrm{tooth} = 64 \Delta v_\textrm{fund}$. Such a population inversion is slightly above the critical threshold in each channel, but the tooth separation is such that each of the 11 discrete samples evolves independently. The transient response of Figure \ref{fig:weakcomb_11samples} is, as expected, a decoherent combination of SR transients from each of the 11 discrete samples, each modulated by the natural frequency of their channel velocity.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_AtDens3over1e-6Each_T5e7_ntoothsep64.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_N0Distribution_Weak.png}
    \caption{Top: transient response of the weakly SR comb of 11 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:weakcomb_11samples}
\end{figure}

The transient depicted in Figure \ref{fig:weakcomb_11samples} contains spurious features in the time domain as a consequence of the artificiality of the comb distribution. In the case of independent samples, the comb distribution of 11 samples separated each by $64 \Delta v_\textrm{fund}$ may be constructed in the Fourier domain by the two steps
\begin{enumerate}
    \item \noindent Convolve an infinite train of Dirac delta distributions, separated by $64 \Delta \omega_\textrm{fund}$, with the Fourier transform of the single sample SR response, and
    \item \noindent Multiply the result by a rectangular window function of width $11 \times 64 \Delta \omega_\textrm{fund}$.
\end{enumerate}
In the time domain such operations correspond to multiplying the transient response of a single sample by a train of 64 $\textrm{sinc}$ functions.\footnote{The inverse Fourier transform of the rectangular window is a $\textrm{sinc}$ function; the remainder of this statement is a simple exercise in combining properties of the Fourier transform.} This is the reason for the strongly oscillating response with periodicity $T/64$. We filter out these artifacts for visualisation purposes by superimposing a cubic spline fit over the data, depicted by the smooth solid line in Figure \ref{fig:weakcomb_11samples}. The SR response is clearly apparent.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_AtDens3over2e-6Each_T5e7_ntoothsep32.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_N0Distribution_Weak.png}
    \caption{Top: transient response of the weakly SR comb of 21 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:weakcomb_21samples}
\end{figure}

We next redistribute the initial population inversions across twice as many channels covering the same total velocity width; that is, we simulate 21 samples, each now with initial population inversion $1.5\times {10}^{-6} \textrm{ m}^{-3}$ and separated by $\Delta v_\textrm{tooth} = 32 \Delta v_\textrm{fund}$. The response is shown in Figure \ref{fig:weakcomb_21samples} where a loss of SR is demonstrated in each of the (now) 21 velocity channels: the peak intensity has dramatically reduced by a factor of $\sim \! 5 \times {10}^5$. Each velocity channel has now been reduced in its initial population inversion below the critical threshold necessary to initiate SR and, importantly, the channel separation of $32 \Delta v_\textrm{fund}$ sufficiently insulates the velocity channels from coupling and thereby bunching into coherent groups.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/641Samples_AtDens3over64e-6Each_T5e7_ntoothsep1.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/641Samples_N0Distribution_Weak.png}
    \caption{Top: transient response of the weakly SR comb of 641 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:weakcomb_641samples}
\end{figure}

Finally, we show in Figure \ref{fig:weakcomb_641samples} the extreme terminal case of this experiment wherein the initial population inversion is redistributed across all 641 available velocity channels. The system now enters a different regime of transient response to the step function of the initial inversion; this transient response peaks at an intensity 9 orders of magnitude smaller than the simulation prior of Figure \ref{fig:weakcomb_21samples}, and its profile should be understood as the step response to the onset of initial inversion prior to settling into the steady state maser regime at $\sim \! {10}^7 \textrm{ s}$.

\subsubsection{Second experiment: slightly below the critical threshold}\label{subsubsec:modsrcomb}

We proceed now with a second experiment wherein the starting configuration of 11 samples separated by $\Delta v_\textrm{tooth} = 64 \Delta v_\textrm{fund}$ begins with twice the initial population inversion as that investigated in Section \ref{subsubsec:weaksrcomb}. We expect, of course, that the SR response of the system will survive one more generation of splitting than did the previous system; however, whether the SR response is sustained down to the continuum remains to be seen.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_AtDens6over1e-6Each_T5e7_ntoothsep64.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_N0Distribution_Medium.png}
    \caption{Top: transient response of the moderately SR comb of 11 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:modcomb_11samples}
\end{figure}

Figure \ref{fig:modcomb_11samples} depicts the initial simulation, where each of the 11 samples is more saturated than in Figure \ref{fig:weakcomb_11samples}. As expected, the response is a decoherent combination of stronger SR transients. The cubic spline shows a much greater peak intensity and shorter characteristic time widths (delay of onset of peak intensity and peak intensity duration).

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_AtDens6over2e-6Each_T5e7_ntoothsep32.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_N0Distribution_Medium.png}
    \caption{Top: transient response of the moderately SR comb of 21 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:modcomb_21samples}
\end{figure}

The degree of initial saturation is now sufficient for SR features to survive one generation of splitting. In Figure \ref{fig:modcomb_21samples} the initial population inversion has been redistributed across 21 samples and the SR features remain. The cubic spline demonstrates again the salient SR features of delayed peak intensity onset and ringing, though reduced in peak intensity and elongated in characteristic time widths (as expected).

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/41Samples_AtDens6over4e-6Each_T5e7_ntoothsep16.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/41Samples_N0Distribution_Medium.png}
    \caption{Top: transient response of the moderately SR comb of 41 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:modcomb_41samples}
\end{figure}

Upon the next generation of splitting, however, the SR features are again lost. In Figure \ref{fig:modcomb_41samples} the initial population distribution has been redistributed across 41 samples but, as with the splitting across 21 samples in the experiment of Section \ref{subsubsec:weaksrcomb}, the channel separation remains too wide to facilitate coherent interaction between the teeth of the comb. The system transitions out of the SR regime and behaves similarly to the response of Figure \ref{fig:weakcomb_641samples} if we continue to the terminal case of 641 samples across this same total velocity width.

\subsubsection{Aside: discussion of the sub-critical responses}\label{subsubsec:subcrit_aside}

The results of Sections \ref{subsubsec:weaksrcomb} and \ref{subsubsec:modsrcomb} naturally imply certain potential responses of the system should the initial population inversion be further increased; however, such expectations will be subverted in Section \ref{subsubsec:strongsrcomb}. It is helpful to pause momentarily and discuss them, so that the importance and subtleties of the actual responses demonstrated thereafter in Section \ref{subsubsec:strongsrcomb} may be properly understood.

One reasonable hypothesis is that, as the initial population inversion is smoothly increased, the number of generations of SR retention might correspondingly increase. For example, perhaps a doubling of the initial population inversion of Section \ref{subsubsec:modsrcomb} would yield the retention of SR features beyond the second comb splitting, but a loss of SR features beyond the third splitting. Perhaps, furthermore, such advancement in splitting tolerance would track smoothly with the initial population inversion until some ultimate value at which SR features could be retained all the way down to the continuum limit.

A second reasonable hypothesis is that the splitting tolerance would at first track with an increasing initial population inversion, but that beyond some critical initial population inversion the combs of the teeth would begin to interact with each other at an ultimate splitting generation well above the continuum limit $\Delta v_\textrm{tooth} = \Delta v_\textrm{fund}$. In such a scenario, one would expect the velocity channels to stochastically coagulate into random coherent bunches of some statistical character across the full velocity width, dependent upon the degree to which the initial population inversion exceeds aforementioned critical threshold. Further comb splitting beyond this ultimate generation would thereafter have no effect, as the teeth of the comb would interact over distances much larger than the fine splitting distance. The transient response in the time domain would then be the decoherent combination of SR responses generated by these statistically independent coagulated coherent velocity groups.

We will find next, however, that neither of these expectations are realised when the initial population inversion exceeds a certain threshold.

\subsubsection{Third experiment: above the critical threshold}\label{subsubsec:strongsrcomb}

We now increase the initial population inversion by a factor of only 50\% relative to Section \ref{subsubsec:modsrcomb}, from $6.0\times {10}^{-6} \textrm{ m}^{-3}$ to $9.0\times {10}^{-6} \textrm{ m}^{-3}$. The transient response for the usual first simulation, a comb distribution of 11 samples, is shown in Figure \ref{fig:strongcomb_11samples}.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_AtDens9over1e-6Each_T5e7_ntoothsep64.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/11Samples_N0Distribution_Strong.png}
    \caption{Top: transient response of the strongly SR comb of 11 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:strongcomb_11samples}
\end{figure}

The peak intensity of Figure \ref{fig:strongcomb_11samples} is slightly higher than expected from the theoretical $n^2$ dependency of peak SR intensity upon initial population inversion. Referencing Figure \ref{fig:modcomb_11samples}, we see a $3.9$-fold increase compared to a theoretical multiplier of $(3/2)^2=2.25$. More interesting, however, are the temporal features of Figure \ref{fig:strongcomb_11samples}. Although the peak intensity duration reduction is roughly consistent with theoretical predictions, the delayed onset of peak intensity is almost entirely eliminated. The situation becomes more dramatic as we proceed to further generations of splitting the comb distribution.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_AtDens9over2e-6Each_T5e7_ntoothsep32.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/21Samples_N0Distribution_Strong.png}
    \caption{Top: transient response of the strongly SR comb of 21 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:strongcomb_21samples}
\end{figure}

We next redistribute the initial population inversion across 21 velocity channels, covering the same total velocity width as previously, and simulate the transient response shown in Figure \ref{fig:strongcomb_21samples}. Surprisingly, we observe now only a slight reduction in peak SR intensity which remains near its previous value of Figure \ref{fig:strongcomb_11samples}; furthermore, the temporal duration and delay to peak intensity are further reduced. Both of these results are in contrast to prior experiments, wherein peak intensity dramatically reduced and temporal features elongated in correspondence with the redistribution of initial population inversion over a generation of splitting.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/41Samples_AtDens9over4e-6Each_T5e7_ntoothsep16.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/41Samples_N0Distribution_Strong.png}
    \caption{Top: transient response of the strongly SR comb of 41 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:strongcomb_41samples}
\end{figure}

Figure \ref{fig:strongcomb_41samples} shows the transient response after another successive generation of splitting, where the initial population inversion has now been redistributed across 41 velocity channels covering the same total velocity width. The two unexpected features of the previous simulation continue to present themselves; namely, the peak intensity remains roughly the same (on the order of ${10}^{-18}$) while temporal structure of any kind is all but non-existent. Neither the finite delay to peak intensity nor the finite peak intensity duration demonstrated in the sub-critical experiments (Sections \ref{subsubsec:weaksrcomb} and \ref{subsubsec:modsrcomb}) are sustained here. In this experiment, the process of filling in the velocity distribution appears to be simultaneously sustaining the high peak intensity characteristic of SR while quenching temporal structure.

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/641Samples_AtDens9over64e-6Each_T5e7_ntoothsep1.png}
    \includegraphics[width=1.\columnwidth, trim=0cm 0cm 0cm 0cm, clip]{figs/641Samples_N0Distribution_Strong.png}
    \caption{Top: transient response of the strongly SR comb of 641 discrete samples. Bottom: illustration of the initial population inversions across velocity channels, truncated to approximately one quarter of the full distribution.}
    \label{fig:strongcomb_641samples}
\end{figure}

The transient response continues to be modified in this fashion through successive generations of comb distribution splitting, all the way down to the terminal case where $\Delta v_\textrm{tooth} = \Delta v_\textrm{fund}$. The response of 641 samples distributed across the same total velocity width as previous simulations is shown in Figure \ref{fig:strongcomb_641samples}: the amplitude of peak intensity remains on the same order of magnitude as previously, while its delay and duration have collapsed.

\section{Continuum Distributions and Transient Structure}\label{sec:cont}

\subsection{Swept pumping mechanism}\label{subsec:cont-swept}

\subsubsection{Interpretations}\label{subsubsec:cont-swept-interp}

The finite temporal duration in the transient response of Figure \ref{fig:strongcomb_641samples} is found, by further simulation, to be inversely proportional to the width of the rectangular plateau defining the velocity distribution. The distribution of Section \ref{subsubsec:strongsrcomb} was a smooth plateau of width $5.8 \times {10}^{-7} \textrm{ m/s}$; doubling that plateau width to $11.6 \times {10}^{-7} \textrm{ m/s}$ while retaining the same spectral density of initial population inversion\footnote{that is, initiating the system with the same population inversion per unit velocity; i.e., with twice the total initial population inversion across the doubly wide velocity distribution} yields a transient response of half the duration of Figure \ref{fig:strongcomb_641samples}. Further simulations continue to show that the duration is inversely proportional to the total velocity width, decreasing indefinitely as the velocity distribution is broadened.

This behaviour of temporal duration with increasing velocity distribution width would be mathematically expected of a collection of independent SR systems prepared with a well-defined polarisation phase relationship. The superposition of identical responses initially in phase and modulated by a continuum of differing Doppler frequencies would interfere to create a Sinc-like total electric field response; this is a familiar result from Fourier analysis.

Such a response is not a priori expected, however, from a system prepared with initially decoherent polarisations, as was indeed the case in each experiment of Section \ref{subsec:comb_distribution}. Were the SR samples composing the velocity distribution truly independent, a distribution prepared with random initial polarisation phases across velocity channels would interfere so as to produce a noise-modulated electric field transient proportional to that of an individual sample's isolated response. A low-pass filter on the intensity would then reproduce the smooth transient SR response, with its finite delay to peak intensity and its finite peak intensity duration, and with a peak intensity scaling linearly with the number of samples in decoherent combination.

We expected, of course, that the 641 velocity channels simulated in Figure \ref{fig:strongcomb_641samples} would not behave truly independently. The channels are coupled in accordance with the results of Section \ref{subsec:two_distrn}, which provide a rough velocity channel interaction distance estimate of $\sim \! 23 \Delta v_\textrm{fund}$. Applying this distance to the second hypothesis of Section \ref{subsubsec:subcrit_aside}, we might have expected a decoherent superposition of SR responses generated by coherent velocity channel bunches of size on the order of 23 channels. We might have hypothesized that such velocity channel groups would develop phase correlations between their polarisations and, as a consequence, have generated a peak intensity of slightly reduced duration (on the order of $T/23$); however, in such a scenario the decoherent combination of transient responses generated by said bunches would sustain temporal structure down to at least some finite duration.

Figure \ref{fig:strongcomb_641samples} demonstrates, however, that beyond the critical threshold no such superposition of statistically independent transient processes emerges. Instead, all transient processes generated within the velocity distribution emerge in a well-defined coherent phase relationship such that temporal structure is quenched in the total field transient. Under the widely Doppler broadened MB equation model of SR, the salient temporal features of SR cannot be sustained by a smooth velocity distribution.

\subsubsection{Stochastic distributions}\label{susubsec:cont-swept-noise}

\subsubsection{Realistic limits to arbitrary temporal quenching}\label{subsubsec:cont-swept-limits}

Some realistic limiting factors should be added to the discussion of Section \ref{subsec:comb_distribution} and to statements made regarding SR in the wide velocity limit. The result of Figure \ref{fig:strongcomb_641samples} and the discussion of Section \ref{subsec:quenching} importantly establish the loss of transient SR structure in the continuum limit, but should not be further extrapolated to conclude the feasibility of arbitrarily fast transient electric field pulse generation. The short temporal duration visible near the start of Figure \ref{fig:strongcomb_641samples} will not realistically decrease indefinitely with increasing velocity distribution width.

Recall from Section \ref{subsec:initial_qm_of_MBeqns} that an initial population inversion is augmented in our model with randomised initial polarisation prescribed by the statistical analysis of the system's initial purely quantum mechanical evolution. That analysis determines a time $\tau_\textrm{classical}$ at which the initial polarisation is established and after which the MB equations may be evolved semi-classically. Importantly, $\tau_\textrm{classical}$ is much smaller than any of the temporal SR features (delay to peak intensity or peak intensity duration) under consideration. We have therefore reasonably assigned the initial polarisation at the start ($\tau=0$) of every simulation rather than at $\tau_\textrm{classical}$; however, this renders our simulations invalid for any processes on times scales of order $\tau_\textrm{classical}$.

Furthermore, at shorter timescales the processes generating the initial population inversion should be accounted for. The transients of Sections \ref{subsubsec:weaksrcomb}, \ref{subsubsec:modsrcomb}, and \ref{subsubsec:strongsrcomb} are step responses to the instantaneous onsets of population inversions, and the sharp pulse near $\tau=0$ may be considered a discontinuity artifact. Conversely, if we smoothly pump the population inversion from zero to its initial value over a small but finite time interval, the quenching of temporal structure by the broad velocity distribution causes the electric field response to track in lockstep with the pumping action; additionally, no overshoot results.

These details at small timescales are not of interest to the present work, which is concerned only with criteria for a system to sustain the finite temporal features of SR in the wide velocity distribution limit. Thus far we have demonstrated the loss of said structure, and it is assumed that a deeper analysis could provide a quantitative description of largely saturated, wide velocity bandwidth responses to transient pumping processes at small timescales. However, we are interested in the following sections as to what characteristics of a system may allow it to demonstrate long timescale SR features and avoid the collapse to lockstep tracking with other short timescale processes within the system.

ADD HERE THE IMPLEMENTATION OF THIS LIMIT VIA THE SF ALGORITHM

\subsection{Transverse pumping mechanism}\label{subsec:cont-trans}

\subsubsection{Autoregulation of finite timescales via the correlation length}\label{subsubsec:cont-trans-autoreg}

\subsection{Thresholds and phase transitions in polarisation transients}\label{subsec:thresholds}

Equipped with the efficiency of the SF algorithm and its ability to suppress distribution edge artifacts by implementing PDC, we are now in a position to simulate the deep interior of a realistic velocity distribution and investigate the mechanisms by which SR temporal features are quenched in widely Doppler broadened samples. The physical intuition gained from this analysis will help us propose and simulate candidate configurations for restoring said features in Section \ref{sec:cont_distr_sustaining}.

We shift now from intensity transients to focus upon polarisation transients across all velocity channels. Polarisation phase relationships tell us about the formation of correlation across the velocity distribution which, in turn, is responsible for the quenching of temporal structure. This is a familiar result from standard Fourier analysis: if the same slow transient $f(t)$ is modulated by a continuum distribution of phase-correlated envelopes, the superposition is inversely proportional in temporal duration to the width of the distribution; for example, identically phased oscillations of $f(t)$ across a continuum of frequencies with width $\Delta \omega$ yield
\begin{align}
    \int_{-\Delta \omega /2}^{\Delta \omega / 2} f(t) e^{-i \omega t} \mathrm{d\omega} &= f(t) \int_{-\Delta \omega /2}^{\Delta \omega / 2} e^{-i \omega t} \mathrm{d\omega} \\
    &= f(t) \Delta \omega \textrm{sinc}\left(\frac{\Delta \omega t}{2}\right).
\end{align}
Applying this simple result to our investigation of sustaining SR temporal features, if a continuum of Doppler offset molecules is to generate a transient SR pulse of finite delay and/or duration, it must do so by a decoherent combination of such a process occurring within independent subgroups of the full distribution. The typical width of each of said subgroups will determine the width of the total transient SR pulse resulting from the superposition of their generated fields.

The velocity channel polarisation phases with PDC form a topology which admits a natural visualisation surface. The polarisation phases on $[0, 2\pi)$ roll over at $2\pi \rightarrow 0$ and the velocity channels on $[v_\textrm{min}, v_\textrm{max}]$ under PDC are connected at $v_\textrm{max} \rightarrow v_\textrm{min}$, so that the two dimensional $(\textrm{polarisation phase}) \times (\textrm{velocity channel})$ surface is topologically equivalent to the $\mathrm{U}(1) \times \mathrm{U}(1) \equiv \mathbb{T}^2$ torus. We therefore plot the polarisation evolution of all velocity channels in every simulation below on $\mathbb{T}^2$. The symmetry across velocity channels, introduced by the Doppler shifted envelopes $\bar{\mathcal{P}}_v$ and by the PDC, implies that no velocity channel possesses special status in our simulations. We thus do not identify either the $v=0$ nor the $v_\textrm{max} \rightarrow v_\textrm{min}$ rollover locations on any torus (apart from Figure \ref{fig:torus_AboveSRnonrot} when we leave the Doppler shifted frames). Similarly, no particular polarisation phase possesses special status when all channels are randomly initialised, and we thus do not identify the location $\angle \bar{\mathcal{P}}_v = 0$ on any torus. The choice of $\mathbb{T}^2$ axis assignment to velocity channels and polarisation phases is labelled on Figure \ref{fig:torus_weak}.

We investigate the polarisation phase transients for initial population inversion levels similar to those used in the earlier experiments of Sections \ref{subsubsec:weaksrcomb}, \ref{subsubsec:modsrcomb}, and \ref{subsubsec:strongsrcomb}. We build upon the final continuum cases of each of those sections' experiments, but now with a wider total velocity distribution width and with PDC implemented via the SF algorithm. In comparing to the results of those prior sections, we ensure that our initial population inversions match as densities in velocity space; i.e., we apply similar initial population inversions per velocity differential, but a larger total population inversion proportional to the total distribution width increase.

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/Weakest/atdens_1e-4_nsch1280nint80_tdur5e7_time0e7.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/Weakest/atdens_1e-4_nsch1280nint80_tdur5e7_time1e7.png}
    \caption{TBD.}
    \label{fig:torus_weak}
\end{figure}

Our first simulation investigates the polarisation phase behaviour well below any transition threshold, starting with a total population inversion of $10^{-4} \textrm{ m}^{-3}$ across 2561 velocity channels, or a density in velocity space of
\begin{equation}
    \frac{10^{-4} \textrm{ m}^{-3}}{2561 dv} = \frac{10^{-4} \textrm{ m}^{-3} \omega_0 T}{2561 c 2 \pi} = 43.6 \textrm{ m}^{-3} / (\textrm{m/s}).
\end{equation}
The response, shown on $\mathbb{T}^2$ in Figure \ref{fig:torus_weak}, is trivial. The left torus displays the polarisation phase distribution at the start of the simulation and the right torus after $10^{7}$ seconds. The scatter points drift only slightly throughout the simulation and develop no correlations. Keeping in mind that the polarisations $\bar{\mathcal{P}}_v$ each define the evolution of Doppler offset fast rotating envelopes, the behaviour depicted in Figure \ref{fig:torus_weak} is that of completely independent velocity channels oscillating independently at their own natural Doppler shifted frequencies. The apparent stationary behaviour is only a result of the variation in factorisation envelope frequency by velocity channel in the definitions of equation \eqref{eq:p_doppler_defn}, and in fact neighbouring channels precess by $2\pi$ relative to each other over the full simulation duration $T$.

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/MedA/atdens_2e-4_nsch1280nint80_tdur5e7_time1e5.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedA/atdens_2e-4_nsch1280nint80_tdur5e7_time2e5.png}
    \\
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 0cm, clip]{figs/Tori/MedA/atdens_2e-4_nsch1280nint80_tdur5e7_time3e5.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedA/atdens_2e-4_nsch1280nint80_tdur5e7_time4e5.png}
    \caption{TBD.}
    \label{fig:torus_MedA}
\end{figure}

We proceed to increase the initial population inversion by a factor of 2 to $87.2 \textrm{ m}^{-3} / (\textrm{m/s})$. This level crosses a certain ``phase transition'' threshold signaled by the clear onset of wide phase correlations across channels visible in Figure \ref{fig:torus_MedA}. The initially randomly phased polarisations quickly coalesce into a smooth contour which wraps around the phase axis of $\mathbb{T}^2$ approximately $5$ times. We refer to this number of rotations around the phase axis at the time of correlation onset as the winding number $W$ for a simulation.

Over multiple repeated simulations of a given initial population inversion, the winding number varies about a mean value due to the stochastic nature of the simulation. This can be understood by imagining the polarisation phases coagulating into local correlated groups of velocity channels, each of some characteristic width $\Delta v_\textrm{corr}$. Each group will emerge at a random phase angle. If adjacent groups happen to emerge at very differing phase angles, they will contribute to $W$; but if they happen to emerge at very similar phase angles, they will not contribute to $W$. Proceeding around the velocity axis of $\mathbb{T}^2$ is therefore something of a random walk, with step size on the order of $\Delta v_\textrm{corr}$, and yielding after one revolution a winding number $W$ which–though varying by simulation–is ultimately dictated by $\Delta v_\textrm{corr}$. The mean winding number $W_\textrm{mean}$ is therefore a useful tool for establishing a correlation phase width metric, which we will herein construct as $\Delta v_\textrm{corr} \equiv \Delta v_\textrm{tot} / W_\textrm{mean}$ where $\Delta v_\textrm{tot} \equiv v_\textrm{max} - v_\textrm{min}$.

The simulation of \ref{fig:torus_MedA} was specifically selected for presentation as a case which achieves the mean $W_\textrm{mean}=5$ of the initial population inversion $87.2 \textrm{ m}^{-3} / (\textrm{m/s})$. 


% HIDDEN FIGURE (RESTORE IF NEEDED,
% BUT I FEEL THERE ARE TOO MANY TORI PLOTS):
% \begin{figure}
%     \centering
%     \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/MedB/atdens_3e-4_nsch1280nint80_tdur5e7_time1e5.png}
%     \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedB/atdens_3e-4_nsch1280nint80_tdur5e7_time2e5.png}
%     \\
%     \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 0cm, clip]{figs/Tori/MedB/atdens_3e-4_nsch1280nint80_tdur5e7_time3e5.png}
%     \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedB/atdens_3e-4_nsch1280nint80_tdur5e7_time4e5.png}
%     \caption{TBD.}
%     \label{fig:torus_MedB}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/MedC/atdens_4e-4_nsch1280nint80_tdur5e7_time1e5.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedC/atdens_4e-4_nsch1280nint80_tdur5e7_time2e5.png}
    \\
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 0cm, clip]{figs/Tori/MedC/atdens_4e-4_nsch1280nint80_tdur5e7_time3e5.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/MedC/atdens_4e-4_nsch1280nint80_tdur5e7_time4e5.png}
    \caption{TBD.}
    \label{fig:torus_MedC}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/AboveSR/atdens_4e-3_nsch1280nint320_tdur5e7_time5e4.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/AboveSR/atdens_4e-3_nsch1280nint320_tdur5e7_time10e4.png}
    \\
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 0cm, clip]{figs/Tori/AboveSR/atdens_4e-3_nsch1280nint320_tdur5e7_time15e4.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/AboveSR/atdens_4e-3_nsch1280nint320_tdur5e7_time20e4.png}
    \caption{TBD.}
    \label{fig:torus_AboveSR}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 1cm, clip]{figs/Tori/AboveSR/AboveSRNonRotFrame/atdens_4e-3_nsch1280nint320_tdur5e7_time11e3_nonrot.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/AboveSR/AboveSRNonRotFrame/atdens_4e-3_nsch1280nint320_tdur5e7_time14e3_nonrot.png}
    \\
    \includegraphics[width=.49\columnwidth, trim=2.5cm 1cm 2.75cm 0cm, clip]{figs/Tori/AboveSR/AboveSRNonRotFrame/atdens_4e-3_nsch1280nint320_tdur5e7_time17e3_nonrot.png}
    \includegraphics[width=.49\columnwidth, trim=2cm 1cm 3.25cm 1cm, clip]{figs/Tori/AboveSR/AboveSRNonRotFrame/atdens_4e-3_nsch1280nint320_tdur5e7_time20e3_nonrot.png}
    \caption{TBD.}
    \label{fig:torus_AboveSRnonrot}
\end{figure}

\section{Applications}\label{sec:app}

\section{ARCHIVED TEXT}

A simple choice\footnote{The lowest order polynomial satisfying these constraints would be a cubic, but a quintic enables the enforcement of continuous second derivative and is aesthetically superior.} of $S_\textrm{w}$ is the ``$S$-curve'' defined as
\begin{equation}
    S_\textrm{w}\left(\tau\right) = \begin{cases}
        0 &\tau<0 \\
        \frac{1}{2} + \frac{15}{16} \left(\frac{\tau-w}{w}\right) - \frac{5}{8}\left(\frac{\tau-w}{w}\right)^3 + \frac{3}{16} \left(\frac{\tau-w}{w}\right)^5 &0 \leq \tau < 2w \\
        1 &\tau \geq 2w,
    \end{cases}
\end{equation}
where $w$ is the second fitting parameter. A fit of this form is superimposed on the transient of Figure \ref{fig:sfa_nsch16383_intensity} and provides a peak intensity estimate of $3.23\times 10^{-23} \textrm{ W/}\textrm{m}^2$ at a time of $1.47\times{10}^7 \textrm{ s}$ for the simulation of $32,767$ total velocity channels.

\subsubsection{Noisy exponential decay in the widely Doppler broadened limit}\label{subsubsec:cont-noisysims-expdecay}

I LEARNED LATER THAT THIS PART IS NOT VALID:

The noisy exponential decay in the fourth panel of Figure \ref{fig:sfa_nsch4095_progression} is a more realistic description of the transient response of a smooth, WDB distribution excited above $N_{0\textrm{ crit}}$ at $\tau=0$ than the instantaneous pulse shown, for example, in the bottom panel of Figure \ref{fig:comb_161channels_toothsepdecreasing}. Regardless of how smooth a distribution might appear on the bandwidth scale defined by the sample's saturation,\footnote{that is, the bandwidth of the SR transient process that a coherent sample in the same non-linear SR regime would demonstrate} it must always possess variations at some scale, however fine it may be. Every distribution will therefore demonstrate noisy exponential decay with time constant $T_2 / 2$ when excited above $N_{0\textrm{ crit}}$, similar to the response of the fourth panel of Figure \ref{fig:sfa_nsch4095_progression} but with time delay reducing to zero in the WDB limit as per our remarks of the previous paragraph.

The exponential decay of the endfire intensity is, in fact, unique to our Doppler-shifted representation of the MB equations as follow from the envelope factorisations of equation \eqref{eq:p_doppler_defn}. Conversely, under the literature-conventional non Doppler-shifted representation of the MB equations, the sudden inversion of a noisy velocity distribution produces a Dirac delta-like endfire intensity transient. The discrepancy between these two responses presents us with two natural questions: first, if the representations are mathematically equivalent, why do they yield differing responses? Second, which response is physically accurate?

The answer to both questions lies in a subtle inequivalence between asserting initial conditions in both representations. To understand the discrepancy, suppose we were to generate a nearly sudden inversion via some pumping process. In either representation, we would start with zero population inversion and zero polarisation at $\tau=0$, and operate an extremely fast inversion pump pulse $\Lambda^{(\textrm{N})}$ over a short duration $d\tau$. Simultaneously, we would necessarily operate a polarisation pump $\Lambda^{(\textrm{P})} = d \Lambda^{(\textrm{N})} \sin\left(\theta_0\right)$ in order to realise the initial Bloch tipping angle prescribed by Section \ref{subsec:theory-initialqm}.

We would now face a decision as to which frame to pump a given polarisation channel in. It is most natural to pump on resonance with every velocity channel, which is achieved in our representation by simply using the same pump term $\Lambda^{(\textrm{P})}=d \Lambda^{(\textrm{N})} \sin\left(\theta_0\right)$ on the right side of each $\omega$-instance of equation \eqref{eq:MB_TD_norm-2}. In the non Doppler-shifted literature convention, however, the act of suddenly inverting the sample corresponds to pumping all polarisation channels in the central $\omega_0$ frame; this differs from our representation by a factor of $\exp\left[i(\omega-\omega_0) v \tau / c \right]$ in each channel's pump.

The act of imposing initial conditions on the system can be understood as the limit of reducing the above pumping process to an infinitesimal duration (a Dirac delta-like pump). The pumping processes are non-equivalent between the conventional and the Doppler-shifted representations of the MB equations, so it is thus not unreasonable to find that their Dirac delta limits yield distinct transient responses. This answers our first question; additionally, the Doppler-shifted factorisation results are more physically justified, as we expect the pumping process to pump all velocity channels symmetrically. It would be unnatural, for example, to assume that some far off-centre velocity channel of natural frequency $\omega_0 + \Delta \omega$ should have its polarisation generated by a pump rotating with frequency $\Delta \omega$; we therefore conclude that our results in the Doppler-offset representation are physically valid.

% \end{document}
